Actors in Multi-Sector Transitions -- Discourse Analysis on Hydrogen in Germany

With net-zero emission goals, low-carbon transitions enter a new phase of development, leading to new challenges for policymaking and research. Multiple transitions unfold in parallel across different sectors. This involves a broad range of technologies, while actors engage in increasingly complex discourses. Here, we study the discourses on hydrogen in Germany. Based on the analysis of 179 newspaper articles from 2016 to 2020, we find that a diverse set of actors, including many industry incumbents, speak favorably about hydrogen, emphasizing economic opportunities and its relevance for the energy transition, whereas skeptics highlight its low energy efficiency and expected scarcity. With the help of discourse network analysis, we identify three emerging conflicts around the use, production, and import of hydrogen. We explain these conflicts and the widespread support of incumbents with a conceptual framework that captures the complex interplay of sectoral contexts, specific technologies and actor interests.

==> Files/tab_N_articles_by_actor.tex <==
\begin{longtable}{l*{1}{ccc}}
                &N\_articles\_by\_actor&         &         \\
                &        b&      pct&   cumpct\\
Nationale Wasserstoffstrategie&       35& 6.227758& 6.227758\\
BMBF - Anja Karliczek&       24& 4.270463& 10.49822\\
BMWi - Peter Altmeier&       15& 2.669039& 13.16726\\
VW - Herbert Diess&       14& 2.491103& 15.65836\\
BMU - Svenja Schulze&       11& 1.957295& 17.61566\\
BMWi            &        9& 1.601423& 19.21708\\
EU Kommission   &        8& 1.423488& 20.64057\\
BDI             &        6& 1.067616& 21.70819\\
BDI - Holger Lösch&        6& 1.067616&  22.7758\\
Daimler - Martin Daum (Truck AG)&        6& 1.067616& 23.84342\\
BMU             &        5& .8896797&  24.7331\\
CAR - Ferdinand Dudenhöffer&        5& .8896797& 25.62278\\
Dena            &        5& .8896797& 26.51246\\
Experten        &        5& .8896797& 27.40214\\
Skeptiker, Kritiker&        5& .8896797& 28.29181\\
Airbus - Guillaume Faury&        4& .7117438& 29.00356\\
BMBF            &        4& .7117438&  29.7153\\
BMVI            &        4& .7117438& 30.42705\\
Befürworter     &        4& .7117438& 31.13879\\
EU Kommission - Frans Timmermanns&        4& .7117438& 31.85053\\
FDP - Andreas Pinkwart&        4& .7117438& 32.56228\\
FNB Gas         &        4& .7117438& 33.27402\\
Gegner der Strategie/Kritiker&        4& .7117438& 33.98577\\
IEA             &        4& .7117438& 34.69751\\
Niedersachsen - Stephan Weil&        4& .7117438& 35.40925\\
Amprion - Klaus Kleinekorte&        3& .5338078& 35.94306\\
Arcelor Mittel  &        3& .5338078& 36.47687\\
BMVI - Alexander Dobrindt&        3& .5338078& 37.01068\\
CDU             &        3& .5338078& 37.54448\\
CDU - Günther Nooke&        3& .5338078& 38.07829\\
CDU - Stefan Kaufmann&        3& .5338078&  38.6121\\
Daimler         &        3& .5338078& 39.14591\\
Die Grünen - Ingrid Nestle&        3& .5338078& 39.67972\\
EU Kommission - Kadri Simson&        3& .5338078& 40.21352\\
EU generell     &        3& .5338078& 40.74733\\
Fraunhofer ISE - Christopher Hebling&        3& .5338078& 41.28114\\
Gaswirtschaft   &        3& .5338078& 41.81495\\
Hyundai - Sae-Hoon Kim&        3& .5338078& 42.34875\\
SPD             &        3& .5338078& 42.88256\\
Salzgitter      &        3& .5338078& 43.41637\\
Siemens Energy - Christian Bruch&        3& .5338078& 43.95018\\
TH Regensburg - Michael Sterner&        3& .5338078& 44.48399\\
Thyssenkrupp    &        3& .5338078& 45.01779\\
Umweltszene und Klimaschützer&        3& .5338078&  45.5516\\
Uniper - Andreas Schierenbeck&        3& .5338078& 46.08541\\
Universität Erlangen-Nürnberg - Veronika Grimm&        3& .5338078& 46.61922\\
VDMA            &        3& .5338078& 47.15302\\
Agora Energiewende&        2& .3558719&  47.5089\\
Air Liquide - Benoit Potier&        2& .3558719& 47.86477\\
BDEW            &        2& .3558719& 48.22064\\
BDEW - Kerstin Andreae&        2& .3558719& 48.57651\\
BUND            &        2& .3558719& 48.93238\\
DUH - Dorothee Saar&        2& .3558719& 49.28826\\
DVGW            &        2& .3558719& 49.64413\\
DWV - Werner Diwald&        2& .3558719&       50\\
Daimler - Dieter Zetsche&        2& .3558719& 50.35587\\
Dena - Andreas Kuhlmann&        2& .3558719& 50.71174\\
Die Grünen      &        2& .3558719& 51.06762\\
Die Grünen - Anton Hofreiter&        2& .3558719& 51.42349\\
Die Grünen - Oliver Krischer&        2& .3558719& 51.77936\\
EWE - Stefan Dohler&        2& .3558719& 52.13523\\
FNB Gas - Ralph Bahke&        2& .3558719&  52.4911\\
Fraunhofer ISE  &        2& .3558719& 52.84698\\
Fraunhofer ISE - Tom Smolinka&        2& .3558719& 53.20285\\
GP Joule - Ove Petersen&        2& .3558719& 53.55872\\
H2 Mobility     &        2& .3558719& 53.91459\\
Hamburg - Michael Westhagemann parteilos&        2& .3558719& 54.27046\\
Helmholtz-Institut - Peter Wasserscheid&        2& .3558719& 54.62633\\
Hyundai Motors - Eusin Chung&        2& .3558719& 54.98221\\
McKinsey        &        2& .3558719& 55.33808\\
Nikola - Trevor Milton&        2& .3558719& 55.69395\\
Open Grid Europe&        2& .3558719& 56.04982\\
RWE - Rolf Martin Schmitz&        2& .3558719& 56.40569\\
Robert Schlögl  &        2& .3558719& 56.76157\\
SPD - Andreas Rimkus&        2& .3558719& 57.11744\\
Salzgitter - Volker Hille&        2& .3558719& 57.47331\\
Salzgitter AG - Heinz Jörg Fuhrmann&        2& .3558719& 57.82918\\
Shell-Niederlande - Marjan van Loon&        2& .3558719& 58.18505\\
Thyssenkrupp - Arnd Köfler&        2& .3558719& 58.54093\\
Toyota - Katsuhiko Hirose&        2& .3558719&  58.8968\\
Wind2Gas - Tim Brandt&        2& .3558719& 59.25267\\
Zukunft Erdgas - Timm Kehler&        2& .3558719& 59.60854\\
Zulieferer\Bosch&        2& .3558719& 59.96441\\
Zulieferer\Elring-Klinger - Stefan Wolf&        2& .3558719& 60.32028\\
ABB Marine and Ports - Juha Koskela&        1& .1779359& 60.49822\\
ADAC            &        1& .1779359& 60.67616\\
Acatech         &        1& .1779359& 60.85409\\
Agora Energiewende - Matthias Deutsch&        1& .1779359& 61.03203\\
Alstom          &        1& .1779359& 61.20996\\
Alstom - Schrank&        1& .1779359&  61.3879\\
Arcelor Mittal - Frank Schulz&        1& .1779359& 61.56584\\
Arcelor Mittal - Uwe Braun&        1& .1779359& 61.74377\\
Audi            &        1& .1779359& 61.92171\\
Aurora Energy Research&        1& .1779359& 62.09964\\
Aurora Energy Research - Hanns Koenig&        1& .1779359& 62.27758\\
Avacon          &        1& .1779359& 62.45552\\
Avacon - Angela Brandes&        1& .1779359& 62.63345\\
BASF - Uwe Liebelt&        1& .1779359& 62.81139\\
BDH             &        1& .1779359& 62.98932\\
BDH - Andreas Lücke&        1& .1779359& 63.16726\\
BDI - Carsten Rolle&        1& .1779359&  63.3452\\
BDI - Joachim Lang&        1& .1779359& 63.52313\\
BDL             &        1& .1779359& 63.70107\\
BMW             &        1& .1779359&   63.879\\
BMW - Klaus Fröhlich&        1& .1779359& 64.05694\\
BMZ - Gerd Müller&        1& .1779359& 64.23488\\
BP              &        1& .1779359& 64.41281\\
BUND - Ernst-Christoph Stolper&        1& .1779359& 64.59075\\
BUND - Oliver Powalla&        1& .1779359& 64.76868\\
BUND - Verena Graichen&        1& .1779359& 64.94662\\
Barclays - Lydia Rainforth&        1& .1779359& 65.12456\\
BeeZero - Thomas Schäfer&        1& .1779359& 65.30249\\
Befürworter von H2&        1& .1779359& 65.48043\\
Berater - Berthold Hannes&        1& .1779359& 65.65836\\
Bosch - Carl Arntzen&        1& .1779359&  65.8363\\
Boston Consulting Group&        1& .1779359& 66.01423\\
Breakthrough Energy - Ann Mettler&        1& .1779359& 66.19217\\
Brot für die Welt&        1& .1779359& 66.37011\\
Bundesanstalt für Materialforschung und -prüfung&        1& .1779359& 66.54804\\
CAN             &        1& .1779359& 66.72598\\
CDU - Tilman Kuban&        1& .1779359& 66.90391\\
CEP - Thomas Bystry&        1& .1779359& 67.08185\\
Creavis - Oliver Busch&        1& .1779359& 67.25979\\
DIHK            &        1& .1779359& 67.43772\\
DIHK - Eric Schweitzer&        1& .1779359& 67.61566\\
DLR - Björn Nagel&        1& .1779359& 67.79359\\
DLR - Franz Philipps&        1& .1779359& 67.97153\\
DLR - Johannes Hartmann&        1& .1779359& 68.14947\\
DLR - Josef Kallo&        1& .1779359&  68.3274\\
DLR - Karsten Lemmer&        1& .1779359& 68.50534\\
DLR - Kaspar Andreas Friedrich&        1& .1779359& 68.68327\\
DNR             &        1& .1779359& 68.86121\\
DUH             &        1& .1779359& 69.03915\\
DWV             &        1& .1779359& 69.21708\\
Daimler - Madeleine Herdlitschka&        1& .1779359& 69.39502\\
Daimler - Ola Källenius&        1& .1779359& 69.57295\\
Dena - Christoph Jugel&        1& .1779359& 69.75089\\
Deutsche Akademie für Technikwissenschaften - Thomas Weber&        1& .1779359& 69.92883\\
Deutsche Bank Research - Eric Heymann&        1& .1779359& 70.10676\\
Deutsche Reeder - Ralf Nagel&        1& .1779359&  70.2847\\
Die Bahn - Sabina Jeschke&        1& .1779359& 70.46263\\
Die Grünen - Cem Özdemir&        1& .1779359& 70.64057\\
Die Grünen - Dieter Janecek&        1& .1779359& 70.81851\\
Die Grünen - Frans Untersteller&        1& .1779359& 70.99644\\
Die Grünen - Michael Bloss&        1& .1779359& 71.17438\\
Die Linke - Eva-Maria Schreiber&        1& .1779359& 71.35231\\
E3G - Felix Heilmann&        1& .1779359& 71.53025\\
EEB - Barbara Mariani&        1& .1779359& 71.70819\\
ENBW - Frank Mastiaux&        1& .1779359& 71.88612\\
EU Kommission - Ursula von der Leyen&        1& .1779359& 72.06406\\
EVP Fraktion - Peter Liese&        1& .1779359& 72.24199\\
EWE             &        1& .1779359& 72.41993\\
EWE - Urban Keußen&        1& .1779359& 72.59786\\
EWI             &        1& .1779359&  72.7758\\
EY - Metin Fidan&        1& .1779359& 72.95374\\
Easac           &        1& .1779359& 73.13167\\
Easac - William Gillet&        1& .1779359& 73.30961\\
Enapter         &        1& .1779359& 73.48754\\
Enapter - Sebastian-Justus Schmidt&        1& .1779359& 73.66548\\
Energieagentur NRW - Stefan Garche&        1& .1779359& 73.84342\\
Energy Brainpool&        1& .1779359& 74.02135\\
Eon - Thomas König&        1& .1779359& 74.19929\\
Equinor         &        1& .1779359& 74.37722\\
Erdgas Schwaben - Jens Dammer&        1& .1779359& 74.55516\\
Evonik - Thomas Basten&        1& .1779359&  74.7331\\
FDP - Christoph Hoffmann&        1& .1779359& 74.91103\\
FDP - Hans Ulrich Rülke&        1& .1779359& 75.08897\\
FH Bergisch Gladbach - Stefan Bratzel&        1& .1779359&  75.2669\\
FNB Gas - Alexander Lennemann&        1& .1779359& 75.44484\\
FNB Gas - Inga Posch&        1& .1779359& 75.62278\\
FNB Gas - Thomas Gößmann&        1& .1779359& 75.80071\\
FU Jülich - Detlef Stolten&        1& .1779359& 75.97865\\
First Berlin - Karsten von Blumenthal&        1& .1779359& 76.15658\\
Fraunhofer IKTS - Matthias Jahn&        1& .1779359& 76.33452\\
Fraunhofer IMWS - Ralf Wehrspohn&        1& .1779359& 76.51246\\
Fraunhofer ISI  &        1& .1779359& 76.69039\\
Fraunhofer ISI - Marlene Arens&        1& .1779359& 76.86833\\
Fraunhofer ISI - Till Gnann&        1& .1779359& 77.04626\\
Fraunhofer IWU - Welf-Guntram Drossel&        1& .1779359&  77.2242\\
GE Power AG Mannheim - Henryk Wulf&        1& .1779359& 77.40214\\
GP Joule        &        1& .1779359& 77.58007\\
Gasunie - Han Fennema&        1& .1779359& 77.75801\\
Gazprom         &        1& .1779359& 77.93594\\
GdW - Axel Gedaschko&        1& .1779359& 78.11388\\
Geldmanager - Uwe Zimmer&        1& .1779359& 78.29181\\
Get H2 Nukleus  &        1& .1779359& 78.46975\\
Graforce - Marc Dünow&        1& .1779359& 78.64769\\
Greenpeace      &        1& .1779359& 78.82562\\
Greenpeace Energy&        1& .1779359& 79.00356\\
Greenpeace Energy - Michael Friedrich&        1& .1779359& 79.18149\\
H2 Mobilität Schweiz - Jörg Ackermann&        1& .1779359& 79.35943\\
H21             &        1& .1779359& 79.53737\\
HAW - Werner Beba&        1& .1779359&  79.7153\\
HTKW - Robert Huhn&        1& .1779359& 79.89324\\
Hafenbehörde Rotterdam - Stijn van Els&        1& .1779359& 80.07117\\
Hamburger Hochbahn&        1& .1779359& 80.24911\\
Hamburger Hochbahn - Heinrich Klingenberg&        1& .1779359& 80.42705\\
Hamburger Hochbahn - Henrik Falk&        1& .1779359& 80.60498\\
Horváth & Partners - Dietmar Voggenreiter&        1& .1779359& 80.78292\\
HySolutions - Heinrich Klingenberg&        1& .1779359& 80.96085\\
Hydrogen Council&        1& .1779359& 81.13879\\
Hydrogenious - Daniel Teichmann&        1& .1779359& 81.31673\\
Hydrogenious Technologies - Daniel Teichmann&        1& .1779359& 81.49466\\
Hyundai - Chung Eui-sun&        1& .1779359&  81.6726\\
Hyundai Hydrogen Mobility AG - Mark Freymüller&        1& .1779359& 81.85053\\
IASS - Stefan Stückrad&        1& .1779359& 82.02847\\
IG Metall - Jörg Hofmann&        1& .1779359& 82.20641\\
IHS - Ben Scott &        1& .1779359& 82.38434\\
IOSB            &        1& .1779359& 82.56228\\
ISI Evercore - John Saager&        1& .1779359& 82.74021\\
IfA - Stefan Reindl&        1& .1779359& 82.91815\\
Ines - Sebastian Bleschke&        1& .1779359& 83.09609\\
InnoEnergy - Christian Müller&        1& .1779359& 83.27402\\
Jeremy Rifkin   &        1& .1779359& 83.45196\\
Kawasaki - Taku Hasegawa&        1& .1779359& 83.62989\\
Keyou - Thomas Korn&        1& .1779359& 83.80783\\
Klimaallianz - Christiane Averbeck&        1& .1779359& 83.98577\\
LEE - Rainer Priggen&        1& .1779359&  84.1637\\
LNVG - Rainer Peters&        1& .1779359& 84.34164\\
Leipziger Landrat - Henry Graichen&        1& .1779359& 84.51957\\
MAN             &        1& .1779359& 84.69751\\
MCC - Brigitte Knopf&        1& .1779359& 84.87544\\
Max Planck - Beatriz Roldan, Robert Schlögl&        1& .1779359& 85.05338\\
McKinsey - Bernd Heid&        1& .1779359& 85.23132\\
Mercedes - Jörg Burzer&        1& .1779359& 85.40925\\
Ministerpräsident Japan - Yoshihide Suga&        1& .1779359& 85.58719\\
Monitoringkommission - Löschel Grimm Lenz Staiß&        1& .1779359& 85.76512\\
Morgan Stanley  &        1& .1779359& 85.94306\\
NGO Menschenrechte Kongo&        1& .1779359&   86.121\\
NN - Schiffer   &        1& .1779359& 86.29893\\
NOW - Klaus Bonhoff&        1& .1779359& 86.47687\\
Niedersachsen - Bernd Althusmann&        1& .1779359&  86.6548\\
Niedersachsen - Olaf Lies SPD&        1& .1779359& 86.83274\\
Nikola          &        1& .1779359& 87.01068\\
Nikola - Mark Russel&        1& .1779359& 87.18861\\
Nikolaus Schües &        1& .1779359& 87.36655\\
Northern Gas Networks - Dan Sadler&        1& .1779359& 87.54448\\
Nowega          &        1& .1779359& 87.72242\\
Oliver Wyman - Romed Kelp&        1& .1779359& 87.90036\\
Open Grid Europe - Thomas Hüwener&        1& .1779359& 88.07829\\
Panasonic       &        1& .1779359& 88.25623\\
Prognos         &        1& .1779359& 88.43416\\
RWE             &        1& .1779359&  88.6121\\
RWTH Aachen - Walter Leitner&        1& .1779359& 88.79004\\
Ritsumeikan Universität - Jörg Raupach&        1& .1779359& 88.96797\\
Roastom         &        1& .1779359& 89.14591\\
Roland Berger - Markus Baum&        1& .1779359& 89.32384\\
Ruhr-Universität Bochum - Thomas Ernst Müller&        1& .1779359& 89.50178\\
SHS - Tim Hartmann&        1& .1779359& 89.67972\\
SPD - Bernd Westphal&        1& .1779359& 89.85765\\
Schleswig-Holstein Netz AG - Sönke Nissen&        1& .1779359& 90.03559\\
Shell - Vigeveno&        1& .1779359& 90.21352\\
Shell Deutschland - Els van Stijn&        1& .1779359& 90.39146\\
Shell Deutschland - Jens Müller Belau&        1& .1779359&  90.5694\\
Siemens - Armin Schnettler&        1& .1779359& 90.74733\\
Siemens - Florian Bergen&        1& .1779359& 90.92527\\
Siemens - Joe Kaeser&        1& .1779359&  91.1032\\
Steffen Bukold  &        1& .1779359& 91.28114\\
Strom- und Gasnetzbetreiber&        1& .1779359& 91.45907\\
Sunfire - Christian von Olshausen&        1& .1779359& 91.63701\\
Sunfire - Nils Aldag&        1& .1779359& 91.81495\\
TU Chemnitz - Thomas von Unwerth&        1& .1779359& 91.99288\\
Tennet - Manon van Beek&        1& .1779359& 92.17082\\
Tesla - Elon Musk&        1& .1779359& 92.34875\\
Thyssenkrupp - Andreas Goss&        1& .1779359& 92.52669\\
Timm Koch - Autor&        1& .1779359& 92.70463\\
Total - Philippe Sauquet&        1& .1779359& 92.88256\\
Toyota - Alain Uyttenhoven&        1& .1779359&  93.0605\\
Toyota - Johan van Zyl&        1& .1779359& 93.23843\\
Toyota - Takeshi Uchiyamada&        1& .1779359& 93.41637\\
UBA             &        1& .1779359& 93.59431\\
Union Investment&        1& .1779359& 93.77224\\
Uniper - Axel Wietfeld&        1& .1779359& 93.95018\\
Universität Bremen - Torben Stührmann&        1& .1779359& 94.12811\\
Universität Nürnberg-Erlangen - Peter Wasserscheid&        1& .1779359& 94.30605\\
VCI             &        1& .1779359& 94.48399\\
VCI - Christian Kullmann&        1& .1779359& 94.66192\\
VCI - Wolfgang Große-Entrup&        1& .1779359& 94.83986\\
VDA - Hilgegard Müller&        1& .1779359& 95.01779\\
VDE             &        1& .1779359& 95.19573\\
VDI             &        1& .1779359& 95.37367\\
VKU             &        1& .1779359&  95.5516\\
Valliant - Norbert Schiedeck&        1& .1779359& 95.72954\\
Vattenfall - Gunnar Groebler&        1& .1779359& 95.90747\\
Viessmann - Maximilian Viessmann&        1& .1779359& 96.08541\\
Vision          &        1& .1779359& 96.26335\\
Voestalpine     &        1& .1779359& 96.44128\\
Voestalpine - Herbert Eibensteiner&        1& .1779359& 96.61922\\
Voestalpine - Wolfgang Eder&        1& .1779359& 96.79715\\
Vonovia         &        1& .1779359& 96.97509\\
WWF             &        1& .1779359& 97.15302\\
Wasserstoff Botschafter Niederlande - Noé van Hulst&        1& .1779359& 97.33096\\
Weltenergierat - Carsten Rolle&        1& .1779359&  97.5089\\
Westenergie - Katharina Reiche&        1& .1779359& 97.68683\\
Wuppertal Institut&        1& .1779359& 97.86477\\
Wuppertal Institut - Manfred Fischedick&        1& .1779359&  98.0427\\
Zukunft Erdgas  &        1& .1779359& 98.22064\\
Zukunft Erdgas - Stephan Kohler&        1& .1779359& 98.39858\\
Zulieferer\Bosch - Andreas Kufferath&        1& .1779359& 98.57651\\
Zulieferer\Bosch - Markus Heyn&        1& .1779359& 98.75445\\
Zulieferer\Bosch - Volkmar Denner&        1& .1779359& 98.93238\\
Zulieferer\Mahle - Jörg Rückauf&        1& .1779359& 99.11032\\
Zulieferer\Plastic Omnium - Laurent Favre&        1& .1779359& 99.28826\\
Öko Institut    &        1& .1779359& 99.46619\\
Öko Institut - Felix Matthes&        1& .1779359& 99.64413\\
Öko Institut - Peter Kasten&        1& .1779359& 99.82206\\
Ökumenisches Netz Zentralafrika&        1& .1779359&      100\\
Total           &      562&      100&         \\
Observations    &      562&         &         \\
\end{longtable}


==> Files/tab_N_codes_all_actors.tex <==
\begin{longtable}{l*{1}{ccc}}
                &N\_content\_codes\_all&         &         \\
                &        b&      pct&   cumpct\\
GB3a Grün erklärtes Ziel&      146& 6.131877& 6.131877\\
CL1 Wichtig für Energiewende und Klimaschutz&      145& 6.089878& 12.22176\\
PP1 Industriepolitische Chancen&      116& 4.871903& 17.09366\\
AP4f Schwerlast oder Schiene&       99& 4.157917& 21.25157\\
PP3 Politische Rahmenbedingungen anpassen&       90& 3.779924&  25.0315\\
AP4a Industrie  &       74& 3.107938& 28.13944\\
AP1 Verschiedene Anwendungen denkbar&       71&  2.98194& 31.12138\\
AP4b Energiespeicher oder Transport&       69& 2.897942& 34.01932\\
Imp3a Importe sind notwendig&       68& 2.855943& 36.87526\\
AP3a Industrie  &       67& 2.813944& 39.68921\\
CL2 Nötig für vollständige Dekarbonisierung&       67& 2.813944& 42.50315\\
ET5 Nutzung überschüssigen Ökostroms&       67& 2.813944& 45.31709\\
KM4 Skaleneffekte realisieren&       59&  2.47795& 47.79504\\
AP5d Nicht für PKW&       53& 2.225955&   50.021\\
ET3 Hoher Energieverlust&       52& 2.183956& 52.20496\\
AP4e PWK        &       50& 2.099958& 54.30491\\
ET1 Integration erneuerbarer Energien&       44& 1.847963& 56.15288\\
ET4 Erneuerbare Energien Ausbau notwendig&       44& 1.847963& 58.00084\\
AP3d Wärme      &       43& 1.805964&  59.8068\\
KM5 Große Mengen nötig&       43& 1.805964& 61.61277\\
AP4i Verkehr allgemein&       42& 1.763965& 63.37673\\
GB1b Nötig für Markthochlauf&       42& 1.763965&  65.1407\\
KM2 Nutzung bestehenden Gasnetzes&       40& 1.679966& 66.82066\\
PP4 Internationale Dimension berücksichtigen&       40& 1.679966& 68.50063\\
AP3b Energiespeicher oder Transport&       36&  1.51197&  70.0126\\
AP3h Synthetische Kraftstoffe&       33& 1.385972& 71.39857\\
AP3i Verkehr allgemein&       33& 1.385972& 72.78454\\
AP4j Flug und Schiff&       33& 1.385972& 74.17052\\
Imp1b Potenzial für günstige Importe&       33& 1.385972& 75.55649\\
AP3f Schwerlast oder Schiene&       31& 1.301974& 76.85846\\
AP3g Stromerzeugung&       30& 1.259975& 78.11844\\
AP4h Synthetische Kraftstoffe&       30& 1.259975& 79.37841\\
AP3j Flug und Schiff&       29& 1.217976& 80.59639\\
AP5e Prioritär für DDI&       29& 1.217976& 81.81436\\
GB2b Nur grün CO2 frei&       28& 1.175976& 82.99034\\
GB1a Verschiedene Farben berücksichtigen&       27& 1.133977& 84.12432\\
AP4c Beimischung Gasnetz&       26& 1.091978&  85.2163\\
AP2 Verschiedene Anwendungen geplant&       25& 1.049979& 86.26627\\
KM1 Perspektivisch günstige Lösung&       25& 1.049979& 87.31625\\
KM3 Grundsätzlich knapp und teuer&       25& 1.049979& 88.36623\\
GB2a Explizit nur grün&       24&  1.00798& 89.37421\\
ETX Hoher Energiebedarf&       23& .9659807& 90.34019\\
GB2d CCS ist umstritten&       22& .9239815& 91.26417\\
AP4d Wärme      &       20& .8399832& 92.10416\\
AP3c Beimischung Gasnetz&       19&  .797984& 92.90214\\
ET2 Technische Schwierigkeiten&       19&  .797984& 93.70013\\
AP5b Effizientere Technologien bevorzugen&       18& .7559849& 94.45611\\
AP3e PKW        &       16& .6719866&  95.1281\\
Imp1c Vorteile für Exporteure&       15& .6299874& 95.75808\\
Imp2a Nachteile für Exporteure&       14& .5879882& 96.34607\\
Imp2b Importabhängigkeit&       13& .5459891& 96.89206\\
AP5c Nicht für Gebäudewärme&       12& .5039899& 97.39605\\
GB1d Nur grün teuer und riskant&       12& .5039899& 97.90004\\
AP4g Stromerzeugung&       11& .4619908& 98.36203\\
GB1c Nur grün nicht möglich&       10& .4199916& 98.78202\\
CL3 Blick auf andere Klimaschutzmaßnahmen wichtig&        9& .3779924& 99.16002\\
GB2c Nicht grün verlängert fossile Energienutzung&        8& .3359933& 99.49601\\
GB1aa Inklusive grau&        5& .2099958& 99.70601\\
PP2 Erhöht Akzeptanz von Energiewende&        4& .1679966&   99.874\\
AP5a Beimischung Gasnetz Verschwendung&        3& .1259975&      100\\
Total           &     2381&      100&         \\
Observations    &     2381&         &         \\
r               &       60&         &         \\
\end{longtable}


==> Files/tab_N_codes_per_article.tex <==
\begin{longtable}{l*{1}{ccc}}
                &N\_codes\_per\_article&         &         \\
                &        b&      pct&   cumpct\\
73\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       42& 1.763965& 1.763965\\
33\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       38& 1.595968& 3.359933\\
Der Wasserstoff bleibt ein Zankapfel&       35& 1.469971& 4.829903\\
Die EU entdeckt den Wasserstoff&       35& 1.469971& 6.299874\\
58\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       34& 1.427971& 7.727845\\
17\_PDFsam\_DIZ PDB\_1&       28& 1.175976& 8.903822\\
108\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       26& 1.091978&   9.9958\\
38\_PDFsam\_DIZ PDB\_1&       26& 1.091978& 11.08778\\
66\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       26& 1.091978& 12.17976\\
Ein Stoff macht Karriere;Um die Wirtschaft CO2-neutral zu mache&       25& 1.049979& 13.22974\\
79\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       24&  1.00798& 14.23772\\
Heilt Wasserstoff das Klima\_;Wasserstoff ist derzeit als angebl&       24&  1.00798&  15.2457\\
Wasserstoff soll die Energiewende retten&       24&  1.00798& 16.25367\\
Wie klimavertr\_glich ist Wasserstoff wirklich\_&       24&  1.00798& 17.26165\\
47\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       23& .9659807& 18.22764\\
55\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       23& .9659807& 19.19362\\
45\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       22& .9239815&  20.1176\\
60\_PDFsam\_DIZ PDB\_1&       22& .9239815& 21.04158\\
Die gr\_ne Begegnung der nachhaltigen Art;Wasserstoff oder Strom&       22& .9239815& 21.96556\\
Neuer Eckpfeiler der deutschen Energiewende;Der Bund plant den&       22& .9239815& 22.88954\\
96\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       21& .8819824& 23.77152\\
So wird Wasserstoff gr\_n;Bei der Energiewende setzt die Politik&       21& .8819824& 24.65351\\
\_H\_ wie Hoffnung;Das Element Wasserstoff kann helfen, Energie e&       21& .8819824& 25.53549\\
99\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       20& .8399832& 26.37547\\
Gr\_ne fordern Pflichtquoten f\_r gr\_nen Stahl&       20& .8399832& 27.21546\\
Herkulesaufgabe Wasserstoffimport&       20& .8399832& 28.05544\\
Wasserstoff f\_r die Energiewende;Die Regierung legt ihre lang e&       20& .8399832& 28.89542\\
1\_PDFsam\_DIZ PDB\_1&       19&  .797984& 29.69341\\
Wasserstoff soll Europas schmutzige Industrien sauber machen;Di&       19&  .797984& 30.49139\\
14\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       18& .7559849& 31.24738\\
17\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       18& .7559849& 32.00336\\
20\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       18& .7559849& 32.75934\\
Der Wasserstoff, aus dem die Tr\_ume sind;Deutschland will bei s&       18& .7559849& 33.51533\\
33\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       17& .7139857& 34.22932\\
53\_PDFsam\_DIZ PDB\_1&       17& .7139857&  34.9433\\
Abl\_sung des Hochofens;Das Unternehmen Salzgitter treibt den Ei&       17& .7139857& 35.65729\\
Ein Sicherheitsnetz f\_r die Energiewende&       17& .7139857& 36.37127\\
Im Wasserstoffrausch&       17& .7139857& 37.08526\\
Windstrom zu Wasserstoff&       17& .7139857& 37.79924\\
42\_PDFsam\_DIZ PDB\_1&       16& .6719866& 38.47123\\
43\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       16& .6719866& 39.14322\\
48\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       16& .6719866&  39.8152\\
Energiebranche setzt auf Tausendsassa Wasserstoff&       16& .6719866& 40.48719\\
Im Wind stecken gro\_e Energiereserven;Das Ideal der Energietech&       16& .6719866& 41.15918\\
Wasserstoff wird ausgebremst&       16& .6719866& 41.83116\\
36\_PDFsam\_DIZ PDB\_2&       15& .6299874& 42.46115\\
40\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       15& .6299874& 43.09114\\
41\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       15& .6299874& 43.72113\\
Die neue Farbenlehre der Energiewende&       15& .6299874& 44.35111\\
Gib Stoff       &       15& .6299874&  44.9811\\
VW klammert sich an das Elektro-Dogma;Der Konzern will zum Mark&       15& .6299874& 45.61109\\
Wasserstoff-Einigung&       15& .6299874& 46.24108\\
15\_PDFsam\_DIZ PDB\_1&       14& .5879882& 46.82906\\
37\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       14& .5879882& 47.41705\\
88\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       14& .5879882& 48.00504\\
Wasserstoff-\_ra r\_ckt n\_her;Ein deutsches Start-up hat kleine G&       14& .5879882& 48.59303\\
102\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       13& .5459891& 49.13902\\
106\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       13& .5459891& 49.68501\\
112\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       13& .5459891&   50.231\\
15\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       13& .5459891& 50.77698\\
36\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       13& .5459891& 51.32297\\
56\_PDFsam\_DIZ PDB\_1&       13& .5459891& 51.86896\\
82\_PDFsam\_DIZ PDB\_1&       13& .5459891& 52.41495\\
90\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       13& .5459891& 52.96094\\
Brennraum statt Zelle&       13& .5459891& 53.50693\\
Skepsis bei der Energie der Zukunft;Das Wirtschaftsministerium&       13& .5459891& 54.05292\\
Viessmann setzt auf Wasserstoff&       13& .5459891& 54.59891\\
2 Milliarden Euro f\_r Wasserstofftechnik&       12& .5039899&  55.1029\\
31\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       12& .5039899& 55.60689\\
92\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       12& .5039899& 56.11088\\
Kein gr\_nes Gas f\_r Heizungen\_;Nationale Wasserstoffstrategie v&       12& .5039899& 56.61487\\
Neue Aufgabe f\_r alte Gasnetze;Wo heute noch Erdgas str\_mt, sol&       12& .5039899& 57.11886\\
24\_PDFsam\_DIZ PDB\_1&       11& .4619908& 57.58085\\
30\_PDFsam\_DIZ PDB\_1&       11& .4619908& 58.04284\\
50\_PDFsam\_DIZ PDB\_1&       11& .4619908& 58.50483\\
83\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       11& .4619908& 58.96682\\
Ein Klassiker kommt in Fahrt;Wasserstoff ist ein altbekannter E&       11& .4619908& 59.42881\\
Im Wasserstoff-Fieber&       11& .4619908&  59.8908\\
Nordwesten wird Modellregion f\_r Wasserstoff&       11& .4619908& 60.35279\\
Trommler f\_r den Wasserstoff&       11& .4619908& 60.81478\\
Wasserstoff ist gut - aber schwer einzuf\_hren&       11& .4619908& 61.27677\\
Wir m\_ssen bei Wasserstoff die Nummer 1 in der Welt werden&       11& .4619908& 61.73877\\
101\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       10& .4199916& 62.15876\\
52\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       10& .4199916& 62.57875\\
55\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       10& .4199916& 62.99874\\
62\_PDFsam\_Genios\_Dokumente\_20210414\_1017&       10& .4199916& 63.41873\\
6\_PDFsam\_Genios\_Dokumente\_20210414\_1020&       10& .4199916& 63.83872\\
Antrieb Wasserstoff;Schwarze Ministerin f\_r gr\_nen Wasserstoff&       10& .4199916& 64.25871\\
Unter der Erde schlummert der wei\_e Schatz;Um Verkehr und Indus&       10& .4199916& 64.67871\\
Wasserstoff statt Diesel\_;Der Abgas-Skandal ersch\_ttert Deutsch&       10& .4199916&  65.0987\\
Windstrom zu speichern ist effizient, aber teuer;Deutschland ha&       10& .4199916& 65.51869\\
12\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        9& .3779924& 65.89668\\
17\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        9& .3779924& 66.27467\\
26\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        9& .3779924& 66.65267\\
30\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        9& .3779924& 67.03066\\
46\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        9& .3779924& 67.40865\\
47\_PDFsam\_DIZ PDB\_1&        9& .3779924& 67.78664\\
50\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        9& .3779924& 68.16464\\
63\_PDFsam\_DIZ PDB\_1&        9& .3779924& 68.54263\\
70\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        9& .3779924& 68.92062\\
8\_PDFsam\_DIZ PDB\_2&        9& .3779924& 69.29861\\
Abgeh\_ngt beim Wasserstoff;Volkswagen, BMW und Daimler haben ak&        9& .3779924& 69.67661\\
Eine Alternative zum Koksen&        9& .3779924&  70.0546\\
Fl\_chtige Tr\_ume&        9& .3779924& 70.43259\\
Heizen mit Wasserstoff;Die Gasheizung wurde als Ursache von Emi&        9& .3779924& 70.81058\\
Nationale Wasserstoffstrategie ignoriert Autos fast v\_llig;Im S&        9& .3779924& 71.18858\\
Plan zur Rettung des Motors;Deutscher \_kostrom reicht nicht aus&        9& .3779924& 71.56657\\
Weg vom \_lhahn;L\_ckenf\_ller Solar- und Windstrom l\_sst sich dez&        9& .3779924& 71.94456\\
Wenn der Wind bl\_st;Die Raffinerie der H&amp;R \_lwerke Schindle&        9& .3779924& 72.32255\\
Wo die Batterie floppt, springt Wasserstoff ein;In Deutschland&        9& .3779924& 72.70055\\
Wundermittel Wasserstoff&        9& .3779924& 73.07854\\
\_Massive Emissionsminderung in allen Sektoren\_&        9& .3779924& 73.45653\\
104\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        8& .3359933& 73.79252\\
115\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        8& .3359933& 74.12852\\
19\_PDFsam\_DIZ PDB\_2&        8& .3359933& 74.46451\\
28\_PDFsam\_DIZ PDB\_1&        8& .3359933&  74.8005\\
28\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        8& .3359933&  75.1365\\
30\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        8& .3359933& 75.47249\\
41\_PDFsam\_DIZ PDB\_2&        8& .3359933& 75.80848\\
4\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        8& .3359933& 76.14448\\
53\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        8& .3359933& 76.48047\\
58\_PDFsam\_DIZ PDB\_1&        8& .3359933& 76.81646\\
Das bezahlbare Wasserstoffauto;Toyota will die Produktion des M&        8& .3359933& 77.15246\\
F\_r Stahl ist das eine Perspektive ;heute auf zoom&        8& .3359933& 77.48845\\
Jahrhundert-Chance oder \_ko-Tr\_umerei\_;Die Aktien von Wassersto&        8& .3359933& 77.82444\\
Milliardenmarkt Wasserstoff&        8& .3359933& 78.16044\\
Spatenstich f\_r Wasserstoff-Tankstelle;27 Triebwagen sollen in&        8& .3359933& 78.49643\\
Streit um die Wasserstoff-Idee;Volkswagen-Chef Herbert Diess gl&        8& .3359933& 78.83242\\
Voestalpine setzt auf Wasserstoff&        8& .3359933& 79.16842\\
Wasserstoff wird zur Chance f\_r Anleger;Risikofreudigen Sparern&        8& .3359933& 79.50441\\
Wirtschaft Kompakt;United-Internet\_ Neue Allianz f\_r 5G-Ausbau&        8& .3359933&  79.8404\\
24\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        7& .2939941&  80.1344\\
26\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        7& .2939941& 80.42839\\
2\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        7& .2939941& 80.72239\\
2\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        7& .2939941& 81.01638\\
35\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        7& .2939941& 81.31037\\
4\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        7& .2939941& 81.60437\\
9\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        7& .2939941& 81.89836\\
Airbus plant mit Wasserstoff;Der Flugzeugbauer setzt bei der En&        7& .2939941& 82.19236\\
Airbus-Chef sieht in E-Autos eine Mogelpackung;Europas Flugzeug&        7& .2939941& 82.48635\\
Die Suche nach der blauen Alternative;Bei der IAA dreht sich sc&        7& .2939941& 82.78034\\
Ein Mann brennt f\_r Wasserstoff;Heinrich Klingenberg hat bei de&        7& .2939941& 83.07434\\
Gr\_nes Gas im Chemiepark;Gut Ding braucht bekanntlich Weile. So&        7& .2939941& 83.36833\\
In J\_lich geht die Supersonne auf;150 Hochleistungsstrahler lie&        7& .2939941& 83.66233\\
\_Die Klima-Bewegung wird immer kompromissloser\_&        7& .2939941& 83.95632\\
\_Wasserstoff ins Erdgas mischen\_&        7& .2939941& 84.25031\\
22\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        6&  .251995& 84.50231\\
7\_PDFsam\_DIZ PDB\_1&        6&  .251995&  84.7543\\
7\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        6&  .251995&  85.0063\\
EEG-Umlage soll \_schnellstm\_glich\_ weg&        6&  .251995& 85.25829\\
Eine Frage      &        6&  .251995& 85.51029\\
Fahren mit Selbstgebranntem&        6&  .251995& 85.76228\\
Linde steigt ins Carsharing-Gesch\_ft ein;Gasekonzern will Wasse&        6&  .251995& 86.01428\\
Oben ohne       &        6&  .251995& 86.26627\\
Streit \_ber Wasserstoff;Die Bundesregierung verschiebt abermals&        6&  .251995& 86.51827\\
Warum nicht Brennstoffzelle\_&        6&  .251995& 86.77026\\
Wasserstoff soll gr\_n werden;Ein Innovationsbeauftragter soll d&        6&  .251995& 87.02226\\
\_Krise hei\_t nicht Entlassung, sondern Verantwortung\_&        6&  .251995& 87.27425\\
22\_PDFsam\_DIZ PDB\_1&        5& .2099958& 87.48425\\
31\_PDFsam\_DIZ PDB\_2&        5& .2099958& 87.69425\\
4\_PDFsam\_DIZ PDB\_2&        5& .2099958& 87.90424\\
Blo\_ nicht noch mal vergeigen!;Kommentar von Bernhard P\_tter zu&        5& .2099958& 88.11424\\
Der Kampf um die Wasserstoff-Heizung&        5& .2099958& 88.32423\\
Der Treibstoff der Zukunft;Forscher und Unternehmen testen Wass&        5& .2099958& 88.53423\\
Deutsche Energiewende auf Kosten Afrikas;Mit Wasserkraft aus de&        5& .2099958& 88.74423\\
Die Energiewende beginnt im Wasserglas;Weltrekord bei der solar&        5& .2099958& 88.95422\\
Die Stahlproduktion soll gr\_ner werden&        5& .2099958& 89.16422\\
Es reicht gerade f\_r die deutsche Stahlindustrie ;G\_nter Nooke,&        5& .2099958& 89.37421\\
Gr\_ner Stahl;F\_r die treibhausgasintensive traditionelle Produk&        5& .2099958& 89.58421\\
Ohne E-Fuels drohe das Job-Desaster;Wirtschaft attackiert Umwel&        5& .2099958&  89.7942\\
Wasser im Tank  &        5& .2099958&  90.0042\\
12\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        4& .1679966&  90.1722\\
14\_PDFsam\_DIZ PDB\_1&        4& .1679966& 90.34019\\
28\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        4& .1679966& 90.50819\\
30\_PDFsam\_DIZ PDB\_2&        4& .1679966& 90.67619\\
35\_PDFsam\_DIZ PDB\_1&        4& .1679966& 90.84418\\
39\_PDFsam\_DIZ PDB\_2&        4& .1679966& 91.01218\\
42\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        4& .1679966& 91.18018\\
4\_PDFsam\_DIZ PDB\_1&        4& .1679966& 91.34817\\
69\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        4& .1679966& 91.51617\\
6\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        4& .1679966& 91.68417\\
75\_PDFsam\_DIZ PDB\_1&        4& .1679966& 91.85216\\
85\_PDFsam\_DIZ PDB\_1&        4& .1679966& 92.02016\\
94\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        4& .1679966& 92.18816\\
9\_PDFsam\_DIZ PDB\_1&        4& .1679966& 92.35615\\
Brennstoffzelle besiegt Tesla und Elektro-Audi;Eine Studie des&        4& .1679966& 92.52415\\
Der Stoff, aus dem die Tr\_ume sind;Von Lukas Weber&        4& .1679966& 92.69215\\
Der blaue Weg;Viele betrachten das Elektroauto als einzige Opti&        4& .1679966& 92.86014\\
Der fl\_ssige Akku&        4& .1679966& 93.02814\\
Die Reichweite ist kein Hemmnis;Batteriefahrzeuge stellen erheb&        4& .1679966& 93.19614\\
Elefantenrennen &        4& .1679966& 93.36413\\
Gas, Alkohol und Steine;An Stromspeichern wird unerm\_dlich gefo&        4& .1679966& 93.53213\\
Mit Wasserstoff zur W\_rmewende;Der Heizungshersteller Vaillant&        4& .1679966& 93.70013\\
Wirtschaft Kompakt;Tarifrunde\_ IG Metall verzichtet auf Geld-Fo&        4& .1679966& 93.86812\\
Wirtschaft plant Wasserstoffnetz&        4& .1679966& 94.03612\\
10\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        3& .1259975& 94.16212\\
12\_PDFsam\_DIZ PDB\_2&        3& .1259975& 94.28811\\
26\_PDFsam\_DIZ PDB\_1&        3& .1259975& 94.41411\\
64\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        3& .1259975& 94.54011\\
6\_PDFsam\_DIZ PDB\_2&        3& .1259975& 94.66611\\
Ammoniak als Treibstoff;Forscher pr\_fen Nutzbarkeit f\_r Elektro&        3& .1259975&  94.7921\\
Anschub f\_r das Wasserstoffauto;Bis 2026 investiert der Bund 25&        3& .1259975&  94.9181\\
Chemieriese ohne Futter;Wenn es nach den Beschl\_ssen der Kohlek&        3& .1259975&  95.0441\\
Deutsch-franz\_sische Wasserstoff-Kooperation&        3& .1259975&  95.1701\\
Eine Frage der Kosten;Wasserstoffautos sind eine saubere Altern&        3& .1259975& 95.29609\\
Gr\_ner Treibstoff aus der Klosch\_ssel;Neue Technik soll Abwasse&        3& .1259975& 95.42209\\
Japan f\_rdert Wasserstoff mit Milliardenpaket&        3& .1259975& 95.54809\\
Japan prescht voran beim Ausbau der Wasserstoff-Tankstellen;Auc&        3& .1259975& 95.67409\\
Japan setzt auf Wasserstoff und Kohle&        3& .1259975& 95.80008\\
Lastwagen mit Wasserstoff im Tank&        3& .1259975& 95.92608\\
Neuer Antrieb f\_r die Bahn&        3& .1259975& 96.05208\\
Vattenfall schaltet erneuerbaren Energien den Turbo zu&        3& .1259975& 96.17808\\
Warum Wasserstoff gegen den E-Motor chancenlos ist;Ist das Elek&        3& .1259975& 96.30407\\
Wasserstoff in neuen Dimensionen;In Niedersachsen entsteht die&        3& .1259975& 96.43007\\
Wasserstofftransport noch unklar&        3& .1259975& 96.55607\\
Wohin geht die Reise\_;Batterie und Brennstoffzelle k\_nnten sich&        3& .1259975& 96.68207\\
Zeitenwende f\_r die Stahlindustrie&        3& .1259975& 96.80806\\
111\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        2& .0839983& 96.89206\\
19\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        2& .0839983& 96.97606\\
1\_PDFsam\_DIZ PDB\_2&        2& .0839983& 97.06006\\
24\_PDFsam\_DIZ PDB\_2&        2& .0839983& 97.14406\\
24\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        2& .0839983& 97.22806\\
33\_PDFsam\_DIZ PDB\_1&        2& .0839983& 97.31205\\
50\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        2& .0839983& 97.39605\\
65\_PDFsam\_DIZ PDB\_1&        2& .0839983& 97.48005\\
67\_PDFsam\_DIZ PDB\_1&        2& .0839983& 97.56405\\
80\_PDFsam\_DIZ PDB\_1&        2& .0839983& 97.64805\\
8\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        2& .0839983& 97.73205\\
Airbus will mit Wasserstoff fliegen&        2& .0839983& 97.81604\\
Bosch setzt auf Brennstoffzelle;Kooperation mit Nikola Motors f&        2& .0839983& 97.90004\\
Bosch setzt auf die Brennstoffzelle&        2& .0839983& 97.98404\\
Der erste Hauptsatz der Energierevolution;Lasst Batterien sprec&        2& .0839983& 98.06804\\
Deutsche Forscher arbeiten am Wasserstoffflieger&        2& .0839983& 98.15204\\
Great Wall und die deutsche Brennstoffzelle&        2& .0839983& 98.23604\\
Hybrit macht Stahl gr\_n;Noch sind Schwedens Stahlwerke die gr\_\_&        2& .0839983& 98.32003\\
Idee\_ Erst leihen, dann kaufen;Mobilit\_t Gase-Hersteller Linde&        2& .0839983& 98.40403\\
In Teterow lebt der Markt&        2& .0839983& 98.48803\\
OMV setzt auf Wasserstoff&        2& .0839983& 98.57203\\
SUV und doch ein gutes Gewissen;Der Hyundai Nexo f\_hrt mit eine&        2& .0839983& 98.65603\\
Schottland will Wasserstoff voranbringen&        2& .0839983& 98.74003\\
Siemens setzt in G\_rlitz jetzt auch auf Wasserstoff;Konzern pla&        2& .0839983& 98.82402\\
Stoff zum Tr\_umen(2)&        2& .0839983& 98.90802\\
Wettlauf um den Elektroantrieb&        2& .0839983& 98.99202\\
\_Wir werden nicht alles mit Strom l\_sen k\_nnen\_&        2& .0839983& 99.07602\\
28\_PDFsam\_DIZ PDB\_2&        1& .0419992& 99.11802\\
34\_PDFsam\_DIZ PDB\_2&        1& .0419992& 99.16002\\
40\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        1& .0419992& 99.20202\\
58\_PDFsam\_Genios\_Dokumente\_20210414\_1020&        1& .0419992& 99.24402\\
6\_PDFsam\_DIZ PDB\_1&        1& .0419992& 99.28601\\
73\_PDFsam\_DIZ PDB\_1&        1& .0419992& 99.32801\\
7\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        1& .0419992& 99.37001\\
86\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        1& .0419992& 99.41201\\
98\_PDFsam\_Genios\_Dokumente\_20210414\_1017&        1& .0419992& 99.45401\\
Aus dem Auspuff kommt nur hei\_e Luft;Verbrennungsmotoren, die m&        1& .0419992& 99.49601\\
Die Alternativen;Bisher haben weniger als zwei Prozent aller Au&        1& .0419992& 99.53801\\
Ende der Bahn-Stinker;Alstom pr\_sentiert den ersten Wasserstoff&        1& .0419992& 99.58001\\
Laborsteak im Klimahaus&        1& .0419992& 99.62201\\
Nikola prescht mit Wasserstoff-Lastern vor&        1& .0419992& 99.66401\\
Nur hei\_e Luft;Der Verkehrsminister will Wasserstoff-Autos f\_rd&        1& .0419992& 99.70601\\
Regionalbahnen in Hessen fahren bald mit Wasserstoff&        1& .0419992& 99.74801\\
Stahlindustrie entdeckt Wasserstoff;Unternehmen forschen an L\_s&        1& .0419992&    99.79\\
Technischer Vorsprung;Japan setzt auf wasserstoffgetriebene Fah&        1& .0419992&   99.832\\
Und was ist mit Wasserstoff\_&        1& .0419992&   99.874\\
Wasserstoff aus dem Elektro-Ofen&        1& .0419992&   99.916\\
Wasserstoff f\_r die Verkehrswende&        1& .0419992&   99.958\\
\_Wir verpassen den Zug nicht noch mal\_;RWE-Chef Rolf Martin Sch&        1& .0419992&      100\\
Total           &     2381&      100&         \\
Observations    &     2381&         &         \\
r               &      266&         &         \\
\end{longtable}


==> Files/tab_N_content_codes_per_actor.tex <==
\begin{longtable}{l*{1}{ccc}}
                &N\_cont\_codes\_per\_actor&         &         \\
                &        b&      pct&   cumpct\\
Frankfurter Allgemeine Zeitung&      238&   9.9958&   9.9958\\
Handelsblatt    &      234& 9.827803&  19.8236\\
Sueddeutsche Zeitung&      128& 5.375892&  25.1995\\
Die Welt        &      123& 5.165897& 30.36539\\
Nationale Wasserstoffstrategie&      115& 4.829903&  35.1953\\
BMBF - Anja Karliczek&      106& 4.451911& 39.64721\\
taz             &       81& 3.401932& 43.04914\\
BMWi - Peter Altmeier&       36&  1.51197& 44.56111\\
BMU - Svenja Schulze&       35& 1.469971& 46.03108\\
EU Kommission - Frans Timmermanns&       28& 1.175976& 47.20706\\
EU Kommission   &       26& 1.091978& 48.29903\\
Amprion - Klaus Kleinekorte&       24&  1.00798& 49.30701\\
FDP - Andreas Pinkwart&       22& .9239815&   50.231\\
VW - Herbert Diess&       22& .9239815& 51.15498\\
BMWi            &       21& .8819824& 52.03696\\
Max Planck - Beatriz Roldan, Robert Schlögl&       20& .8399832& 52.87694\\
Niedersachsen - Stephan Weil&       19&  .797984& 53.67493\\
BDI             &       18& .7559849& 54.43091\\
Westenergie - Katharina Reiche&       16& .6719866&  55.1029\\
RWE - Rolf Martin Schmitz&       15& .6299874& 55.73289\\
Universität Erlangen-Nürnberg - Veronika Grimm&       14& .5879882& 56.32087\\
Airbus - Guillaume Faury&       13& .5459891& 56.86686\\
BUND - Verena Graichen&       12& .5039899& 57.37085\\
Daimler - Martin Daum (Truck AG)&       12& .5039899& 57.87484\\
Fraunhofer ISE - Tom Smolinka&       12& .5039899& 58.37883\\
Klimaallianz - Christiane Averbeck&       12& .5039899& 58.88282\\
Robert Schlögl  &       12& .5039899& 59.38681\\
BDI - Holger Lösch&       11& .4619908&  59.8488\\
Befürworter     &       11& .4619908& 60.31079\\
CDU - Günther Nooke&       11& .4619908& 60.77278\\
CDU - Stefan Kaufmann&       11& .4619908& 61.23478\\
Die Grünen - Ingrid Nestle&       11& .4619908& 61.69677\\
GP Joule - Ove Petersen&       11& .4619908& 62.15876\\
Viessmann - Maximilian Viessmann&       11& .4619908& 62.62075\\
Die Grünen - Dieter Janecek&       10& .4199916& 63.04074\\
EU Kommission - Kadri Simson&       10& .4199916& 63.46073\\
EWE - Stefan Dohler&       10& .4199916& 63.88072\\
VDMA            &       10& .4199916& 64.30071\\
DWV - Werner Diwald&        9& .3779924& 64.67871\\
Dena            &        9& .3779924&  65.0567\\
Experten        &        9& .3779924& 65.43469\\
Gegner der Strategie/Kritiker&        9& .3779924& 65.81268\\
Hamburg - Michael Westhagemann parteilos&        9& .3779924& 66.19068\\
Hyundai - Sae-Hoon Kim&        9& .3779924& 66.56867\\
Siemens - Florian Bergen&        9& .3779924& 66.94666\\
Siemens Energy - Christian Bruch&        9& .3779924& 67.32465\\
Tennet - Manon van Beek&        9& .3779924& 67.70265\\
Zukunft Erdgas - Timm Kehler&        9& .3779924& 68.08064\\
BMU             &        8& .3359933& 68.41663\\
BUND - Oliver Powalla&        8& .3359933& 68.75262\\
Dena - Andreas Kuhlmann&        8& .3359933& 69.08862\\
FNB Gas         &        8& .3359933& 69.42461\\
IEA             &        8& .3359933&  69.7606\\
Prognos         &        8& .3359933&  70.0966\\
Skeptiker, Kritiker&        8& .3359933& 70.43259\\
CAR - Ferdinand Dudenhöffer&        7& .2939941& 70.72659\\
Helmholtz-Institut - Peter Wasserscheid&        7& .2939941& 71.02058\\
Hyundai Motors - Eusin Chung&        7& .2939941& 71.31457\\
NN - Schiffer   &        7& .2939941& 71.60857\\
SPD - Andreas Rimkus&        7& .2939941& 71.90256\\
Salzgitter - Volker Hille&        7& .2939941& 72.19656\\
Shell Deutschland - Els van Stijn&        7& .2939941& 72.49055\\
TH Regensburg - Michael Sterner&        7& .2939941& 72.78454\\
Timm Koch - Autor&        7& .2939941& 73.07854\\
Total - Philippe Sauquet&        7& .2939941& 73.37253\\
Uniper - Axel Wietfeld&        7& .2939941& 73.66653\\
Voestalpine - Wolfgang Eder&        7& .2939941& 73.96052\\
Wind2Gas - Tim Brandt&        7& .2939941& 74.25451\\
Agora Energiewende&        6&  .251995& 74.50651\\
Agora Energiewende - Matthias Deutsch&        6&  .251995&  74.7585\\
BDEW            &        6&  .251995&  75.0105\\
Berater - Berthold Hannes&        6&  .251995& 75.26249\\
DIHK            &        6&  .251995& 75.51449\\
DUH - Dorothee Saar&        6&  .251995& 75.76648\\
EU generell     &        6&  .251995& 76.01848\\
Hamburger Hochbahn - Heinrich Klingenberg&        6&  .251995& 76.27047\\
IG Metall - Jörg Hofmann&        6&  .251995& 76.52247\\
Monitoringkommission - Löschel Grimm Lenz Staiß&        6&  .251995& 76.77446\\
Toyota - Katsuhiko Hirose&        6&  .251995& 77.02646\\
Uniper - Andreas Schierenbeck&        6&  .251995& 77.27845\\
Zukunft Erdgas  &        6&  .251995& 77.53045\\
Zulieferer\Bosch - Volkmar Denner&        6&  .251995& 77.78244\\
BMBF            &        5& .2099958& 77.99244\\
BMVI - Alexander Dobrindt&        5& .2099958& 78.20244\\
Befürworter von H2&        5& .2099958& 78.41243\\
DLR - Karsten Lemmer&        5& .2099958& 78.62243\\
DVGW            &        5& .2099958& 78.83242\\
Fraunhofer ISE  &        5& .2099958& 79.04242\\
Fraunhofer ISE - Christopher Hebling&        5& .2099958& 79.25241\\
Hafenbehörde Rotterdam - Stijn van Els&        5& .2099958& 79.46241\\
InnoEnergy - Christian Müller&        5& .2099958& 79.67241\\
Nikola - Mark Russel&        5& .2099958&  79.8824\\
RWTH Aachen - Walter Leitner&        5& .2099958&  80.0924\\
Ruhr-Universität Bochum - Thomas Ernst Müller&        5& .2099958& 80.30239\\
Salzgitter      &        5& .2099958& 80.51239\\
Thyssenkrupp    &        5& .2099958& 80.72239\\
Zulieferer\Elring-Klinger - Stefan Wolf&        5& .2099958& 80.93238\\
Arcelor Mittel  &        4& .1679966& 81.10038\\
BDH             &        4& .1679966& 81.26837\\
BMVI            &        4& .1679966& 81.43637\\
BUND            &        4& .1679966& 81.60437\\
CDU - Tilman Kuban&        4& .1679966& 81.77236\\
CEP - Thomas Bystry&        4& .1679966& 81.94036\\
DIHK - Eric Schweitzer&        4& .1679966& 82.10836\\
DWV             &        4& .1679966& 82.27635\\
Daimler         &        4& .1679966& 82.44435\\
Die Grünen - Anton Hofreiter&        4& .1679966& 82.61235\\
Die Grünen - Michael Bloss&        4& .1679966& 82.78034\\
E3G - Felix Heilmann&        4& .1679966& 82.94834\\
Easac           &        4& .1679966& 83.11634\\
GE Power AG Mannheim - Henryk Wulf&        4& .1679966& 83.28433\\
Gaswirtschaft   &        4& .1679966& 83.45233\\
Gazprom         &        4& .1679966& 83.62033\\
GdW - Axel Gedaschko&        4& .1679966& 83.78832\\
Get H2 Nukleus  &        4& .1679966& 83.95632\\
H2 Mobility     &        4& .1679966& 84.12432\\
HySolutions - Heinrich Klingenberg&        4& .1679966& 84.29231\\
Hydrogenious Technologies - Daniel Teichmann&        4& .1679966& 84.46031\\
Morgan Stanley  &        4& .1679966& 84.62831\\
Nikolaus Schües &        4& .1679966&  84.7963\\
Open Grid Europe - Thomas Hüwener&        4& .1679966&  84.9643\\
RWE             &        4& .1679966&  85.1323\\
Salzgitter AG - Heinz Jörg Fuhrmann&        4& .1679966& 85.30029\\
Shell-Niederlande - Marjan van Loon&        4& .1679966& 85.46829\\
Thyssenkrupp - Arnd Köfler&        4& .1679966& 85.63629\\
Toyota - Takeshi Uchiyamada&        4& .1679966& 85.80428\\
Umweltszene und Klimaschützer&        4& .1679966& 85.97228\\
VCI - Christian Kullmann&        4& .1679966& 86.14028\\
VKU             &        4& .1679966& 86.30827\\
Valliant - Norbert Schiedeck&        4& .1679966& 86.47627\\
WWF             &        4& .1679966& 86.64427\\
Wasserstoff Botschafter Niederlande - Noé van Hulst&        4& .1679966& 86.81226\\
Wuppertal Institut&        4& .1679966& 86.98026\\
BASF - Uwe Liebelt&        3& .1259975& 87.10626\\
BDEW - Kerstin Andreae&        3& .1259975& 87.23226\\
BDH - Andreas Lücke&        3& .1259975& 87.35825\\
BDI - Carsten Rolle&        3& .1259975& 87.48425\\
BMZ - Gerd Müller&        3& .1259975& 87.61025\\
BP              &        3& .1259975& 87.73625\\
Barclays - Lydia Rainforth&        3& .1259975& 87.86224\\
Bosch - Carl Arntzen&        3& .1259975& 87.98824\\
Breakthrough Energy - Ann Mettler&        3& .1259975& 88.11424\\
CDU             &        3& .1259975& 88.24024\\
Creavis - Oliver Busch&        3& .1259975& 88.36623\\
DLR - Björn Nagel&        3& .1259975& 88.49223\\
DLR - Franz Philipps&        3& .1259975& 88.61823\\
DUH             &        3& .1259975& 88.74423\\
Deutsche Bank Research - Eric Heymann&        3& .1259975& 88.87022\\
Deutsche Reeder - Ralf Nagel&        3& .1259975& 88.99622\\
Die Grünen      &        3& .1259975& 89.12222\\
Die Grünen - Oliver Krischer&        3& .1259975& 89.24822\\
EEB - Barbara Mariani&        3& .1259975& 89.37421\\
EVP Fraktion - Peter Liese&        3& .1259975& 89.50021\\
Energieagentur NRW - Stefan Garche&        3& .1259975& 89.62621\\
Eon - Thomas König&        3& .1259975&  89.7522\\
FDP - Hans Ulrich Rülke&        3& .1259975&  89.8782\\
FNB Gas - Ralph Bahke&        3& .1259975&  90.0042\\
GP Joule        &        3& .1259975&  90.1302\\
Graforce - Marc Dünow&        3& .1259975& 90.25619\\
Greenpeace      &        3& .1259975& 90.38219\\
Horváth & Partners - Dietmar Voggenreiter&        3& .1259975& 90.50819\\
MCC - Brigitte Knopf&        3& .1259975& 90.63419\\
McKinsey        &        3& .1259975& 90.76018\\
McKinsey - Bernd Heid&        3& .1259975& 90.88618\\
NOW - Klaus Bonhoff&        3& .1259975& 91.01218\\
Niedersachsen - Olaf Lies SPD&        3& .1259975& 91.13818\\
Nikola - Trevor Milton&        3& .1259975& 91.26417\\
Open Grid Europe&        3& .1259975& 91.39017\\
Panasonic       &        3& .1259975& 91.51617\\
SPD             &        3& .1259975& 91.64217\\
SPD - Bernd Westphal&        3& .1259975& 91.76816\\
Strom- und Gasnetzbetreiber&        3& .1259975& 91.89416\\
VDA - Hilgegard Müller&        3& .1259975& 92.02016\\
Vision          &        3& .1259975& 92.14616\\
Zulieferer\Bosch&        3& .1259975& 92.27215\\
Zulieferer\Plastic Omnium - Laurent Favre&        3& .1259975& 92.39815\\
Air Liquide - Benoit Potier&        2& .0839983& 92.48215\\
Arcelor Mittal - Uwe Braun&        2& .0839983& 92.56615\\
Audi            &        2& .0839983& 92.65015\\
Aurora Energy Research&        2& .0839983& 92.73415\\
BMW - Klaus Fröhlich&        2& .0839983& 92.81814\\
Daimler - Dieter Zetsche&        2& .0839983& 92.90214\\
Deutsche Akademie für Technikwissenschaften - Thomas Weber&        2& .0839983& 92.98614\\
Die Bahn - Sabina Jeschke&        2& .0839983& 93.07014\\
Die Grünen - Cem Özdemir&        2& .0839983& 93.15414\\
ENBW - Frank Mastiaux&        2& .0839983& 93.23814\\
EU Kommission - Ursula von der Leyen&        2& .0839983& 93.32213\\
EWE             &        2& .0839983& 93.40613\\
EWI             &        2& .0839983& 93.49013\\
Enapter         &        2& .0839983& 93.57413\\
Energy Brainpool&        2& .0839983& 93.65813\\
Equinor         &        2& .0839983& 93.74213\\
FH Bergisch Gladbach - Stefan Bratzel&        2& .0839983& 93.82612\\
FNB Gas - Inga Posch&        2& .0839983& 93.91012\\
Fraunhofer IKTS - Matthias Jahn&        2& .0839983& 93.99412\\
Fraunhofer IMWS - Ralf Wehrspohn&        2& .0839983& 94.07812\\
Fraunhofer IWU - Welf-Guntram Drossel&        2& .0839983& 94.16212\\
Gasunie - Han Fennema&        2& .0839983& 94.24612\\
HTKW - Robert Huhn&        2& .0839983& 94.33011\\
Hydrogen Council&        2& .0839983& 94.41411\\
Hydrogenious - Daniel Teichmann&        2& .0839983& 94.49811\\
Hyundai Hydrogen Mobility AG - Mark Freymüller&        2& .0839983& 94.58211\\
IfA - Stefan Reindl&        2& .0839983& 94.66611\\
Ines - Sebastian Bleschke&        2& .0839983&  94.7501\\
Kawasaki - Taku Hasegawa&        2& .0839983&  94.8341\\
Keyou - Thomas Korn&        2& .0839983&  94.9181\\
Ministerpräsident Japan - Yoshihide Suga&        2& .0839983&  95.0021\\
Northern Gas Networks - Dan Sadler&        2& .0839983&  95.0861\\
Roastom         &        2& .0839983&  95.1701\\
Roland Berger - Markus Baum&        2& .0839983& 95.25409\\
Shell - Vigeveno&        2& .0839983& 95.33809\\
Siemens - Joe Kaeser&        2& .0839983& 95.42209\\
Thyssenkrupp - Andreas Goss&        2& .0839983& 95.50609\\
Toyota - Johan van Zyl&        2& .0839983& 95.59009\\
VDE             &        2& .0839983& 95.67409\\
VDI             &        2& .0839983& 95.75808\\
Vattenfall - Gunnar Groebler&        2& .0839983& 95.84208\\
Voestalpine - Herbert Eibensteiner&        2& .0839983& 95.92608\\
Zulieferer\Mahle - Jörg Rückauf&        2& .0839983& 96.01008\\
Öko Institut - Felix Matthes&        2& .0839983& 96.09408\\
Öko Institut - Peter Kasten&        2& .0839983& 96.17808\\
ABB Marine and Ports - Juha Koskela&        1& .0419992& 96.22008\\
ADAC            &        1& .0419992& 96.26207\\
Acatech         &        1& .0419992& 96.30407\\
Alstom          &        1& .0419992& 96.34607\\
Alstom - Schrank&        1& .0419992& 96.38807\\
Arcelor Mittal - Frank Schulz&        1& .0419992& 96.43007\\
Aurora Energy Research - Hanns Koenig&        1& .0419992& 96.47207\\
Avacon          &        1& .0419992& 96.51407\\
Avacon - Angela Brandes&        1& .0419992& 96.55607\\
BDI - Joachim Lang&        1& .0419992& 96.59807\\
BDL             &        1& .0419992& 96.64007\\
BMW             &        1& .0419992& 96.68207\\
BUND - Ernst-Christoph Stolper&        1& .0419992& 96.72407\\
BeeZero - Thomas Schäfer&        1& .0419992& 96.76606\\
Boston Consulting Group&        1& .0419992& 96.80806\\
Brot für die Welt&        1& .0419992& 96.85006\\
Bundesanstalt für Materialforschung und -prüfung&        1& .0419992& 96.89206\\
CAN             &        1& .0419992& 96.93406\\
DLR - Johannes Hartmann&        1& .0419992& 96.97606\\
DLR - Josef Kallo&        1& .0419992& 97.01806\\
DLR - Kaspar Andreas Friedrich&        1& .0419992& 97.06006\\
DNR             &        1& .0419992& 97.10206\\
Daimler - Madeleine Herdlitschka&        1& .0419992& 97.14406\\
Daimler - Ola Källenius&        1& .0419992& 97.18606\\
Dena - Christoph Jugel&        1& .0419992& 97.22806\\
Die Grünen - Frans Untersteller&        1& .0419992& 97.27005\\
Die Linke - Eva-Maria Schreiber&        1& .0419992& 97.31205\\
EWE - Urban Keußen&        1& .0419992& 97.35405\\
EY - Metin Fidan&        1& .0419992& 97.39605\\
Easac - William Gillet&        1& .0419992& 97.43805\\
Enapter - Sebastian-Justus Schmidt&        1& .0419992& 97.48005\\
Erdgas Schwaben - Jens Dammer&        1& .0419992& 97.52205\\
Evonik - Thomas Basten&        1& .0419992& 97.56405\\
FDP - Christoph Hoffmann&        1& .0419992& 97.60605\\
FNB Gas - Alexander Lennemann&        1& .0419992& 97.64805\\
FNB Gas - Thomas Gößmann&        1& .0419992& 97.69005\\
FU Jülich - Detlef Stolten&        1& .0419992& 97.73205\\
First Berlin - Karsten von Blumenthal&        1& .0419992& 97.77404\\
Fraunhofer ISI  &        1& .0419992& 97.81604\\
Fraunhofer ISI - Marlene Arens&        1& .0419992& 97.85804\\
Fraunhofer ISI - Till Gnann&        1& .0419992& 97.90004\\
Geldmanager - Uwe Zimmer&        1& .0419992& 97.94204\\
Greenpeace Energy&        1& .0419992& 97.98404\\
Greenpeace Energy - Michael Friedrich&        1& .0419992& 98.02604\\
H2 Mobilität Schweiz - Jörg Ackermann&        1& .0419992& 98.06804\\
H21             &        1& .0419992& 98.11004\\
HAW - Werner Beba&        1& .0419992& 98.15204\\
Hamburger Hochbahn&        1& .0419992& 98.19404\\
Hamburger Hochbahn - Henrik Falk&        1& .0419992& 98.23604\\
Hyundai - Chung Eui-sun&        1& .0419992& 98.27803\\
IASS - Stefan Stückrad&        1& .0419992& 98.32003\\
IHS - Ben Scott &        1& .0419992& 98.36203\\
IOSB            &        1& .0419992& 98.40403\\
ISI Evercore - John Saager&        1& .0419992& 98.44603\\
Jeremy Rifkin   &        1& .0419992& 98.48803\\
LEE - Rainer Priggen&        1& .0419992& 98.53003\\
LNVG - Rainer Peters&        1& .0419992& 98.57203\\
Leipziger Landrat - Henry Graichen&        1& .0419992& 98.61403\\
MAN             &        1& .0419992& 98.65603\\
Mercedes - Jörg Burzer&        1& .0419992& 98.69803\\
NGO Menschenrechte Kongo&        1& .0419992& 98.74003\\
Niedersachsen - Bernd Althusmann&        1& .0419992& 98.78202\\
Nikola          &        1& .0419992& 98.82402\\
Nowega          &        1& .0419992& 98.86602\\
Oliver Wyman - Romed Kelp&        1& .0419992& 98.90802\\
Ritsumeikan Universität - Jörg Raupach&        1& .0419992& 98.95002\\
SHS - Tim Hartmann&        1& .0419992& 98.99202\\
Schleswig-Holstein Netz AG - Sönke Nissen&        1& .0419992& 99.03402\\
Shell Deutschland - Jens Müller Belau&        1& .0419992& 99.07602\\
Siemens - Armin Schnettler&        1& .0419992& 99.11802\\
Steffen Bukold  &        1& .0419992& 99.16002\\
Sunfire - Christian von Olshausen&        1& .0419992& 99.20202\\
Sunfire - Nils Aldag&        1& .0419992& 99.24402\\
TU Chemnitz - Thomas von Unwerth&        1& .0419992& 99.28601\\
Tesla - Elon Musk&        1& .0419992& 99.32801\\
Toyota - Alain Uyttenhoven&        1& .0419992& 99.37001\\
UBA             &        1& .0419992& 99.41201\\
Union Investment&        1& .0419992& 99.45401\\
Universität Bremen - Torben Stührmann&        1& .0419992& 99.49601\\
Universität Nürnberg-Erlangen - Peter Wasserscheid&        1& .0419992& 99.53801\\
VCI             &        1& .0419992& 99.58001\\
VCI - Wolfgang Große-Entrup&        1& .0419992& 99.62201\\
Voestalpine     &        1& .0419992& 99.66401\\
Vonovia         &        1& .0419992& 99.70601\\
Weltenergierat - Carsten Rolle&        1& .0419992& 99.74801\\
Wuppertal Institut - Manfred Fischedick&        1& .0419992&    99.79\\
Zukunft Erdgas - Stephan Kohler&        1& .0419992&   99.832\\
Zulieferer\Bosch - Andreas Kufferath&        1& .0419992&   99.874\\
Zulieferer\Bosch - Markus Heyn&        1& .0419992&   99.916\\
Öko Institut    &        1& .0419992&   99.958\\
Ökumenisches Netz Zentralafrika&        1& .0419992&      100\\
Total           &     2381&      100&         \\
Observations    &     2381&         &         \\
\end{longtable}


==> Files/tab_N_content_codes_per_actor_inst.tex <==
\begin{longtable}{l*{1}{ccc}}
                &N\_cont\_codes\_per\_actor\_in&         &         \\
                &        b&      pct&   cumpct\\
Frankfurter Allgemeine Zeitung&      238&   9.9958&   9.9958\\
Handelsblatt    &      234& 9.827803&  19.8236\\
Sueddeutsche Zeitung&      128& 5.375892&  25.1995\\
Die Welt        &      123& 5.165897& 30.36539\\
Nationale Wasserstoffstrategie&      115& 4.829903&  35.1953\\
BMBF            &      111& 4.661907&  39.8572\\
taz             &       81& 3.401932& 43.25913\\
EU Kommission   &       66& 2.771945& 46.03108\\
BMWi            &       57& 2.393952& 48.42503\\
BMU             &       43& 1.805964&   50.231\\
Die Grünen      &       38& 1.595968& 51.82696\\
BDI             &       33& 1.385972& 53.21294\\
CDU             &       29& 1.217976& 54.43091\\
FDP             &       26& 1.091978& 55.52289\\
BUND            &       25& 1.049979& 56.57287\\
Amprion         &       24&  1.00798& 57.58085\\
Niedersachsen   &       23& .9659807& 58.54683\\
Fraunhofer ISE  &       22& .9239815& 59.47081\\
VW              &       22& .9239815& 60.39479\\
Daimler         &       20& .8399832& 61.23478\\
Max Planck      &       20& .8399832& 62.07476\\
RWE             &       19&  .797984& 62.87274\\
Dena            &       18& .7559849& 63.62873\\
Westenergie     &       16& .6719866& 64.30071\\
Zukunft Erdgas  &       16& .6719866&  64.9727\\
FNB Gas         &       15& .6299874& 65.60269\\
DLR             &       14& .5879882& 66.19068\\
GP Joule        &       14& .5879882& 66.77866\\
Universität Erlangen&       14& .5879882& 67.36665\\
Airbus          &       13& .5459891& 67.91264\\
DWV             &       13& .5459891& 68.45863\\
EWE             &       13& .5459891& 69.00462\\
SPD             &       13& .5459891& 69.55061\\
Toyota          &       13& .5459891&  70.0966\\
Uniper          &       13& .5459891& 70.64259\\
Agora Energiewende&       12& .5039899& 71.14658\\
Klimaallianz    &       12& .5039899& 71.65057\\
Robert Schlögl  &       12& .5039899& 72.15456\\
Salzgitter      &       12& .5039899& 72.65855\\
Siemens         &       12& .5039899& 73.16254\\
Befürworter     &       11& .4619908& 73.62453\\
Thyssenkrupp    &       11& .4619908& 74.08652\\
Viessmann       &       11& .4619908& 74.54851\\
Zulieferer\Bosch&       11& .4619908&  75.0105\\
DIHK            &       10& .4199916& 75.43049\\
Hyundai         &       10& .4199916& 75.85048\\
VDMA            &       10& .4199916& 76.27047\\
Voestalpine     &       10& .4199916& 76.69047\\
BDEW            &        9& .3779924& 77.06846\\
BMVI            &        9& .3779924& 77.44645\\
DUH             &        9& .3779924& 77.82444\\
Experten        &        9& .3779924& 78.20244\\
Gegner der Strategie/Kritiker&        9& .3779924& 78.58043\\
Hamburg         &        9& .3779924& 78.95842\\
Nikola          &        9& .3779924& 79.33641\\
Siemens Energy  &        9& .3779924& 79.71441\\
Tennet          &        9& .3779924&  80.0924\\
Hamburger Hochbahn&        8& .3359933& 80.42839\\
IEA             &        8& .3359933& 80.76438\\
Prognos         &        8& .3359933& 81.10038\\
Shell Deutschland&        8& .3359933& 81.43637\\
Skeptiker, Kritiker&        8& .3359933& 81.77236\\
BDH             &        7& .2939941& 82.06636\\
CAR             &        7& .2939941& 82.36035\\
Helmholtz       &        7& .2939941& 82.65435\\
Hyundai Motors  &        7& .2939941& 82.94834\\
NN              &        7& .2939941& 83.24234\\
Open Grid Europe&        7& .2939941& 83.53633\\
TH Regensburg   &        7& .2939941& 83.83032\\
Timm Koch       &        7& .2939941& 84.12432\\
Total           &        7& .2939941& 84.41831\\
Wind2Gas        &        7& .2939941& 84.71231\\
Berater         &        6&  .251995&  84.9643\\
EU generell     &        6&  .251995&  85.2163\\
IG Metall       &        6&  .251995& 85.46829\\
McKinsey        &        6&  .251995& 85.72029\\
Monitoringkommission&        6&  .251995& 85.97228\\
Shell           &        6&  .251995& 86.22428\\
VCI             &        6&  .251995& 86.47627\\
Befürworter von H2&        5& .2099958& 86.68627\\
DVGW            &        5& .2099958& 86.89626\\
Easac           &        5& .2099958& 87.10626\\
Hafenbehörde Rotterdam&        5& .2099958& 87.31625\\
InnoEnergy      &        5& .2099958& 87.52625\\
RWTH Aachen     &        5& .2099958& 87.73625\\
Ruhr            &        5& .2099958& 87.94624\\
Wuppertal Institut&        5& .2099958& 88.15624\\
Zulieferer\Elring&        5& .2099958& 88.36623\\
Öko Institut    &        5& .2099958& 88.57623\\
Arcelor Mittel  &        4& .1679966& 88.74423\\
CEP             &        4& .1679966& 88.91222\\
E3G             &        4& .1679966& 89.08022\\
GE Power AG Mannheim&        4& .1679966& 89.24822\\
Gaswirtschaft   &        4& .1679966& 89.41621\\
Gazprom         &        4& .1679966& 89.58421\\
GdW             &        4& .1679966&  89.7522\\
Get H2 Nukleus  &        4& .1679966&  89.9202\\
H2 Mobility     &        4& .1679966&  90.0882\\
HySolutions     &        4& .1679966& 90.25619\\
Hydrogenious Technologies&        4& .1679966& 90.42419\\
Morgan Stanley  &        4& .1679966& 90.59219\\
Nikolaus Schües &        4& .1679966& 90.76018\\
Salzgitter AG   &        4& .1679966& 90.92818\\
Umweltszene und Klimaschützer&        4& .1679966& 91.09618\\
VKU             &        4& .1679966& 91.26417\\
Valliant        &        4& .1679966& 91.43217\\
WWF             &        4& .1679966& 91.60017\\
Wasserstoff Botschafter Niederlande&        4& .1679966& 91.76816\\
Arcelor Mittal  &        3& .1259975& 91.89416\\
Aurora Energy Research&        3& .1259975& 92.02016\\
BASF            &        3& .1259975& 92.14616\\
BMW             &        3& .1259975& 92.27215\\
BMZ             &        3& .1259975& 92.39815\\
BP              &        3& .1259975& 92.52415\\
Barclays        &        3& .1259975& 92.65015\\
Bosch           &        3& .1259975& 92.77614\\
Breakthrough Energy&        3& .1259975& 92.90214\\
Creavis         &        3& .1259975& 93.02814\\
Deutsche Bank Research&        3& .1259975& 93.15414\\
Deutsche Reeder &        3& .1259975& 93.28013\\
EEB             &        3& .1259975& 93.40613\\
EVP Fraktion    &        3& .1259975& 93.53213\\
Enapter         &        3& .1259975& 93.65813\\
Energieagentur NRW&        3& .1259975& 93.78412\\
Eon             &        3& .1259975& 93.91012\\
Fraunhofer ISI  &        3& .1259975& 94.03612\\
Graforce        &        3& .1259975& 94.16212\\
Greenpeace      &        3& .1259975& 94.28811\\
Horváth & Partners&        3& .1259975& 94.41411\\
MCC             &        3& .1259975& 94.54011\\
NOW             &        3& .1259975& 94.66611\\
Panasonic       &        3& .1259975&  94.7921\\
Strom           &        3& .1259975&  94.9181\\
VDA             &        3& .1259975&  95.0441\\
Vision          &        3& .1259975&  95.1701\\
Zulieferer\Plastic Omnium&        3& .1259975& 95.29609\\
Air Liquide     &        2& .0839983& 95.38009\\
Alstom          &        2& .0839983& 95.46409\\
Audi            &        2& .0839983& 95.54809\\
Avacon          &        2& .0839983& 95.63209\\
Deutsche Akademie für Technikwissenschaften&        2& .0839983& 95.71609\\
Die Bahn        &        2& .0839983& 95.80008\\
ENBW            &        2& .0839983& 95.88408\\
EWI             &        2& .0839983& 95.96808\\
Energy Brainpool&        2& .0839983& 96.05208\\
Equinor         &        2& .0839983& 96.13608\\
FH Bergisch Gladbach&        2& .0839983& 96.22008\\
Fraunhofer IKTS &        2& .0839983& 96.30407\\
Fraunhofer IMWS &        2& .0839983& 96.38807\\
Fraunhofer IWU  &        2& .0839983& 96.47207\\
Gasunie         &        2& .0839983& 96.55607\\
Greenpeace Energy&        2& .0839983& 96.64007\\
HTKW            &        2& .0839983& 96.72407\\
Hydrogen Council&        2& .0839983& 96.80806\\
Hydrogenious    &        2& .0839983& 96.89206\\
Hyundai Hydrogen Mobility AG&        2& .0839983& 96.97606\\
IfA             &        2& .0839983& 97.06006\\
Ines            &        2& .0839983& 97.14406\\
Kawasaki        &        2& .0839983& 97.22806\\
Keyou           &        2& .0839983& 97.31205\\
Ministerpräsident Japan&        2& .0839983& 97.39605\\
Northern Gas Networks&        2& .0839983& 97.48005\\
Roastom         &        2& .0839983& 97.56405\\
Roland Berger   &        2& .0839983& 97.64805\\
Sunfire         &        2& .0839983& 97.73205\\
VDE             &        2& .0839983& 97.81604\\
VDI             &        2& .0839983& 97.90004\\
Vattenfall      &        2& .0839983& 97.98404\\
Zulieferer\Mahle&        2& .0839983& 98.06804\\
ABB Marine and Ports&        1& .0419992& 98.11004\\
ADAC            &        1& .0419992& 98.15204\\
Acatech         &        1& .0419992& 98.19404\\
BDL             &        1& .0419992& 98.23604\\
BeeZero         &        1& .0419992& 98.27803\\
Boston Consulting Group&        1& .0419992& 98.32003\\
Brot für die Welt&        1& .0419992& 98.36203\\
Bundesanstalt für Materialforschung und&        1& .0419992& 98.40403\\
CAN             &        1& .0419992& 98.44603\\
DNR             &        1& .0419992& 98.48803\\
Die Linke       &        1& .0419992& 98.53003\\
EY              &        1& .0419992& 98.57203\\
Erdgas Schwaben &        1& .0419992& 98.61403\\
Evonik          &        1& .0419992& 98.65603\\
FU Jülich       &        1& .0419992& 98.69803\\
First Berlin    &        1& .0419992& 98.74003\\
Geldmanager     &        1& .0419992& 98.78202\\
H2 Mobilität Schweiz&        1& .0419992& 98.82402\\
H21             &        1& .0419992& 98.86602\\
HAW             &        1& .0419992& 98.90802\\
IASS            &        1& .0419992& 98.95002\\
IHS             &        1& .0419992& 98.99202\\
IOSB            &        1& .0419992& 99.03402\\
ISI Evercore    &        1& .0419992& 99.07602\\
Jeremy Rifkin   &        1& .0419992& 99.11802\\
LEE             &        1& .0419992& 99.16002\\
LNVG            &        1& .0419992& 99.20202\\
Leipziger Landrat&        1& .0419992& 99.24402\\
MAN             &        1& .0419992& 99.28601\\
Mercedes        &        1& .0419992& 99.32801\\
NGO Menschenrechte Kongo&        1& .0419992& 99.37001\\
Nowega          &        1& .0419992& 99.41201\\
Oliver Wyman    &        1& .0419992& 99.45401\\
Ritsumeikan Universität&        1& .0419992& 99.49601\\
SHS             &        1& .0419992& 99.53801\\
Schleswig       &        1& .0419992& 99.58001\\
Steffen Bukold  &        1& .0419992& 99.62201\\
TU Chemnitz     &        1& .0419992& 99.66401\\
Tesla           &        1& .0419992& 99.70601\\
UBA             &        1& .0419992& 99.74801\\
Union Investment&        1& .0419992&    99.79\\
Universität Bremen&        1& .0419992&   99.832\\
Universität Nürnberg&        1& .0419992&   99.874\\
Vonovia         &        1& .0419992&   99.916\\
Weltenergierat  &        1& .0419992&   99.958\\
Ökumenisches Netz Zentralafrika&        1& .0419992&      100\\
Total           &     2381&      100&         \\
Observations    &     2381&         &         \\
\end{longtable}


==> Files/tab_storylines_overview_selection.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\begin{table}

\caption{Storyline overview}\label{tab:storyline_test}

\centering

\scriptsize
%\doublespacing
\onehalfspacing

%\renewcommand{\arraystretch}{1}
%\setlength{\tabcolsep}{5pt}

\begin{tabular}{llll}
\hline
\rule{0pt}{3ex}Storyline short & Anzahl & Für Paper & Grund\\ 
\hline
CL1 Important for energy transition & 83 & + & Drin lassen um generelle Attention bzgl H2 nachzuzeichnen \\
CL2 Required for complete decarbonization & 38 & + & Sehr interessant, eine Art Proxy für Klimaneutralitätsdebatte \\
CL3 Consider other mitigation options & 6 & - & Interessant, aber fast nie gecoded, vorhandene Codes schwach, daher raus \\
ET1 Integration of renewables & 16 & + & Ganz interessant, technisches Argument für H2, wenig normativ \\
ET2 Technical difficulties & 3 & - & Selten codiert, schwierig zu kodieren, weil oft technologiespezifisch. Lieber rauslassen \\
ET3 High energy losses & 14 & + & Oft erwähnt, wichtig, definitiv drin lassen \\
ETX High energy demand & 7 & - & Ähnlich zu ET3, aber weniger kritisch. Erste 124 Artikel müssten nachgecoded werden. Lieber rauslassen, Mehrwert+Kosten/Nutzen \\
ET4 More efficient technologies preferred & 9 & + & Wenn auch selten, guter Code, drin lassen, stärker als ET3 \\
ET5 Increase RE deployment & 29 & - & Code okay, aber selten so explizit gesagt wie von Karlizcek. Kodierung öfters schwierig, eher rauslassen. \\
ET6 Use excess renewable electricity & 21 & - & Wird oft im Nebensatz erwähnt, aber mir ist die Bedeutung nicht ganz klar. Würde ihn rauslassen. \\
PP1 Economic opportunities & 95 & + & Eines der stärksten pro-Argumente. Definitiv drin lassen. Ggf. disaggregieren   \\
PP2 Increases acceptance of energy transition & 3 & - & Erwähnen dass kodiert, aber kaum genutzt (4 mal...), rauslassen. \\
PP3 Adjust political conditions & 82 & - & Wichtig, aber schwierig. Tendenz die Koiderung nicht als Storyline zu verwerten, sondern um Politische Debatten nachzuzeichen (EEG Novelle, RED, Gasnetzregulierung, etc.) \\
PP4 Consider international dimension & 36 & + & Interessant genug um es zu erwähnen, aber auch etwas nichtssagend. Erwähnen, aber nicht Fokus \\
KM1 Eventually cheap option & 15 & + & Finde ich gut, weil sehr oft wir auf die (aktuell) hohen Kosten hingewiesen. \\
KM2 Use existing gas grid & 27 & + & Auf jeden Fall drin lassen. Ggf. differenzieren zwischen ``Möglichkeit'' und ``Tolle Option''.  \\
KM3 Generally scarce and expensive & 12 & + & Seltener erwähnt als gedacht, aber wichtiges Gegenargument. \\
KM4 Realize economics of scale & 47 & - & Würde ich rauslassen, da Bedeutung nicht ganz klar. \\
KM5 Large quantities required & 21 & - & Ähnlich wie KM4: Schon interessant, aber keine pro-contra Aussage. Und Sorge dass manchmal Kodierung vergessen :( \\
Imp1a Potentially cheap imports & 20 & + & Aggregieren zu ``Imports beneficial'' . \\
Imp1b Advantage for exporters & 10 & + & Aggregieren zu ``Imports beneficial'' \\
Imp2a Disadvantage for exporters & 10 & + & Aggregieren zu ``Imports concerining'' \\
Imp2b Import dependency & 10 & + & Aggregieren zu ``Imports concerining'' \\
Imp3a Imports required & 41 & + & Drin lassen, zeigt Konsens über generelle Notwendigkeit von Importen \\
GB1a Consider various colors & 25  & + & Aggregieren zu ``non-green necessary''  \\
GB1b Include grey & 5 & + & Aggregieren zu ``non-green necessary'' \\
GB1c Transition and market creation & 33 & + & Aggregieren zu ``non-green necessary'' \\
GB1d Only green not possible & 6 & + & Aggregieren zu ``non-green necessary''  \\
GB1e Only green cheap and risky & 9 & + & Aggregieren zu ``non-green necessary'' \\
GB2a Explicitly green only & 21 & + & Aggregieren zu ``Exclusively green'' \\
GB2b Only green without CO2 & 15 & + & Aggregieren zu ``Exclusively green''  \\
GB2c Not green prolongs fossil fuel use & 6 & + & Aggregieren zu ``Exclusively green'' \\
GB2d CCS is contested & 7 & + & Aggregieren zu ``Exclusively green'' \\
GB3a Green generally envisaged & 109 & + & Eigener Code, zeigt Konsens über ziel \\
AP1 Various applications possible & 17 & + & Code gesetzt, wenn Auflistung möglicher (!) Anwendungen \\
AP2 Broad application envisaged & 7 & + & Explizit Befürworter einer breiten Anwendung \\
AP3ff  & 62 & - & Wenn H2 Anwendung als Teil von Auflistung \\
AP4ff  & ~360 & + & Nutzungen wenn explizit hervorgehoben. Nötig für Gegenüberstellung AP5ff. Abgrenzung zu AP3 teils schwierig.  \\
AP5a Not for gas grid & 3 & + & Alle Folgenden wichtig  \\
AP5b Not for heating & 9 & + & \\
AP5c Not for cars & 42 & + &  \\
AP5d Priority for DDIs & 21  & + &  \\
\end{tabular}
\caption*{\footnotesize Note.
For each storyline, the table shows 
the short version (1$^{st}$ column), 
the long version (2$^{nd}$ column),
and one example quote (3$^{rd}$ column).


}
\end{table}
}
